Implicit Two-Tower Policies

We present a new class of structured reinforcement learning policy-architectures, Implicit Two-Tower (ITT) policies, where the actions are chosen based on the attention scores of their learnable latent representations with those of the input states. By explicitly disentangling action from state processing in the policy stack, we achieve two main goals: substantial computational gains and better performance. Our architectures are compatible with both: discrete and continuous action spaces. By conducting tests on 15 environments from OpenAI Gym and DeepMind Control Suite, we show that ITT-architectures are particularly suited for blackbox/evolutionary optimization and the corresponding policy training algorithms outperform their vanilla unstructured implicit counterparts as well as commonly used explicit policies. We complement our analysis by showing how techniques such as hashing and lazy tower updates, critically relying on the two-tower structure of ITTs, can be applied to obtain additional computational improvements.

==> sections/broader_impact.tex <==
\section{Limitations \& broader impacts of this work}
\label{sec:broader_impact}
Several methods presented in this work can be further extended, potentially providing additional improvements of ITTs. For instance, it seems that splitting the set of action-vectors in the given node of the RFT in such a way that the sets in its children have relatively small diameter (rather than arbitrarily) should improve the overall hierarchical hashing mechanism, yet it is not clear how to do that. 
% Furthermore, we focus in this work on the ES-based training algorithms, yet it would be interesting to test ITTs for a broader range of policy-optimization algorithms, potentially also for $Q$-learning. 
Even though presented methods do not have a direct negative societal impact, RL-policy training should be done responsibly, especially given its potential military applications. % as well as the risk associated with agents exploiting extreme exploration strategies (safety concerns).



